Yang-Mills form factors on self-dual backgrounds

The construction of perturbative quantities on non-linear backgrounds leads to the possibility of incorporating strong field effects in perturbation theory. We continue a programme to construct QFT observables on self-dual backgrounds. The approach works with asymptotic data for fields defined at null infinity $\mathscr{I}$, extending earlier work on Yang-Mills amplitudes on self-dual backgrounds to form factors and incorporating supersymmetry. Since our analysis is based on reconstruction from data at null infinity, it naturally ties into work on celestial and twisted holography. We study form factors both in pure Yang-Mills and their supersymmetric counterparts in $\mathcal{N}=4$ SYM, giving a full treatment of $\mathcal{N}=4$ super-Yang-Mills at null infinity and their self-dual nonlinear backgrounds. We obtain tree-level MHV form factors around these backgrounds using new formulae for lifting operators to twistor space leading to simple dressings of the corresponding form factors around the vacuum. We give brief indications on how to go beyond the MHV sector by introducing dressed versions of the MHV diagram propagator. We discuss generating functionals of the MHV all plus 1-loop amplitude in this context together with its various dual conformal representations.

==> constraint_equations.tex <==
\section{$\N=4$ constraint equations on chiral superspace}\label{app:N=4_constraints}
\emph{\color{red} Remember to adapt the normalization in the EOMs taken from the literature so that they agree with our equations.}
In this section, we show how to derive the $\N=4$ equations of motion for the superfields 
\begin{subequations}
    \begin{eqnarray}
        \unabla_{\dot\alpha}^\beta\uB_{\alpha\beta}&=&\{\utpsi_{a\dot\alpha},\upsi^a_\alpha\}-\frac{1}{2}[\uphi_{ab},\unabla_{\alpha\dot\alpha}\uphi^{ab}]\,,\label{eq:super_B_eom}\\
        \unabla_\alpha^{\dot\alpha}\utpsi_{a\dot\alpha}&=&\lambda[\upsi^b_\alpha,\uphi_{ab}]\,,\label{eq:super_tpsi_eom}\\
        \usquare\uphi_{ab}&=&\{\upsi_{\dot\alpha[a},\upsi^{\dot\alpha}_{b]}\}+\lambda\epsilon_{abcd}\{\upsi^c_\alpha,\upsi^{d\alpha}\}+\lambda[\uphi_{c[a},[\uphi^{cd},\uphi_{b]d}]]\,,\label{eq:super_phi_eom}\\
        \unabla_{\dot\alpha}^\alpha\upsi^a_\alpha&=&[\utpsi_{b\dot\alpha},\uphi^{ab}]\,,\label{eq:super_psi_eom}\\\uF_{\alpha\beta}&=&\lambda \uB_{\alpha\beta}\,,\label{eq:super_F_eom}
    \end{eqnarray}
\end{subequations}
from suitably deformed constraint equations on chiral superspace. Prior to our work, it was known that
\begin{itemize}
    \item it's possible to derive the \emph{self-dual} $\N=4$ SYM equations of motion for the superfields from the constraint equations on chiral superspace \cite{Devchand:1996gv}
    \begin{equation}
        [\underline\nabla_{A(\alpha},\underline\nabla_{\beta)B}\}=0\,,
    \end{equation}
    \item it's possible to derive the \emph{full} $\N=4$ SYM equations of motion for the superfields from the constraint equations for the $d=10$, $\N=1$ SYM theory compactified to four dimensions on \emph{non}-chiral superspace \cite{Witten:1978xx, Harnad:1985bc},
    \item it's possible to reconstruct the \emph{full} $\N=4$ equations of motion for the superfields from the constraint equations on chiral superspace
    \cite{Adamo:2013cra}
    \begin{equation}
        [\underline\nabla_{a(\alpha},\underline\nabla_{\beta)B}\}=0\,,
    \end{equation}
    together with the additional constraints
    \begin{equation}
        \underline\nabla_{\alpha a}\underline\phi_{bc}=\underline\nabla_{\alpha [a}\underline\phi_{bc]}\,,\qquad 2\underline\nabla_{\alpha\dot\alpha}\underline\phi_{ab}=\underline\nabla_{\alpha a}\underline{\tilde\psi}_{b\dot\alpha}
    \end{equation}
    and imposing the equations of motion for the lowest-component fields
    \begin{subequations}
    \begin{eqnarray}
    \nabla^\beta_{\dot\alpha}B_{\alpha\beta}&=&\{\tilde\psi_{a\dot\alpha},\psi^a_\alpha\}-\frac{1}{2}[\phi_{ab},\nabla_{\alpha\dot\alpha}\phi^{ab}]\,,\\
    \nabla_{\dot\alpha}^\alpha\psi_\alpha^a&=&[\tilde\psi_{b\dot\alpha},\phi^{ab}]\,,\\
    \square\phi_{ab}&=&\{\tilde\psi_{\dot\alpha[a},\tilde\psi^{\dot\alpha}_{b]}\}+\lambda\epsilon_{abcd}\{\psi^c_\alpha,\psi^{d\alpha}\}+\lambda[\phi_{c[a},[\phi^{cd},\phi_{b]d}]]\,.
    \end{eqnarray}
    \end{subequations}
\end{itemize}
Here we show instead that it's possible to derive the full $\N=4$ SYM equations of motion for the superfields from the constraint equations on chiral superspace
\begin{subequations}
    \begin{eqnarray}
        [\underline\nabla_{a(\alpha},\underline\nabla_{\beta)B}\}&=&0\,,\label{eq:chiral_constraint}\\
        \underline F_{\alpha\beta}&=&\lambda \underline B_{\alpha\beta}\label{eq:F_B_lagrange_multiplier}\,,
    \end{eqnarray}
\end{subequations}
where $\underline F_{\alpha\beta}$ is the ASD component of the supercurvature $[\underline\nabla_{\alpha\dot\alpha},\underline\nabla_{\beta\dot\beta}]$, $\underline B_{\alpha\beta}$ is determined by the constraint equations \eqref{eq:chiral_constraint} as we explain below, and $\lambda$ is the 't Hooft coupling. Our result is therefore a deformation away from self-duality of the results in \cite{Devchand:1996gv} and reduces to that construction in the $\lambda=0$ limit, and is vastly improved compared to the result of \cite{Adamo:2013cra}.

We begin with the construction of the various superfields appearing in the equations of motion. We first define the supercurvature components as implied by the constraint equations
\begin{subequations}
    \begin{eqnarray}
        [\underline\nabla_{\alpha\dot\alpha},\underline\nabla_{\beta\dot\beta}]&\coloneqq&\varepsilon_{\alpha\beta}\underline{\tilde F}_{\dot\alpha\dot\beta}+\varepsilon_{\dot\alpha\dot\beta}\underline{F}_{\alpha\beta}\,,\label{eq:bb_constraint}\\
        {[\underline\nabla_{\alpha a},\underline\nabla_{\beta\dot\alpha}]}&\coloneqq&\varepsilon_{\alpha\beta}\underline{\tilde\psi}_{\dot\alpha a}\,,\label{eq:bf_constraint}\\\{\underline\nabla_{\alpha a},\underline\nabla_{\beta b}\}&\coloneqq&\varepsilon_{\alpha\beta}\underline\phi_{ab}\,,\label{eq:ff_constraint}
    \end{eqnarray}
\end{subequations}
as well as
\begin{equation}
    \underline\phi^{ab}\coloneqq\frac{1}{2}\epsilon^{abcd}\underline\phi_{cd}\,.
\end{equation}
The Jacobi identity for $\underline\nabla_{\alpha a}$, $\underline\nabla_{\beta b}$, and $\underline\nabla_{\gamma c}$ readily implies 
\begin{equation}
    \underline\nabla_{\alpha a}\underline\phi_{bc}=\underline\nabla_{\alpha[a}\phi_{bc]}\,,
\end{equation}
so that we can define the field
\begin{equation}
    \underline\psi^a_\alpha\coloneqq\frac{1}{3!}\epsilon^{abcd}\underline\nabla_{\alpha b}\underline\phi_{cd}=\frac{1}{3}\underline\nabla_{\alpha b}\underline\phi^{ab}\,.
\end{equation}
Similarly, the constraint equation \eqref{eq:ff_constraint} implies that the superfield
\begin{equation}
    \underline\nabla_{a(\alpha}\underline\nabla_{\beta)b}\phi_{cd}\,,
\end{equation}
is totally skew in the $\SU(4)$ indices, so we define
\begin{equation}
    \underline B_{\alpha\beta}\coloneqq \underline\nabla_{a(\alpha}\psi^a_{\beta)}\,.
\end{equation}
We complete our definition by introducing the 't Hooft coupling $\lambda$ and by requiring
\begin{equation}
    \underline F_{\alpha\beta}=\lambda \underline B_{\alpha\beta}\,,
\end{equation}
for the ASD part of the bosonic supercurvature.

With these definitions, we can derive the $\N=4$ equations of motion as follows: we first consider the equations of motion for $\upsi^a_\alpha$ and $\uB_{\alpha\beta}$ and notice that the Jacobi identity for $\unabla_{\alpha \dot\alpha}$, $\unabla_{\beta b}$, and $\unabla_{\gamma c}$ can be written as
\begin{equation}
2\underline\nabla_{\alpha\dot\alpha}\uphi_{ab}=\unabla_{\alpha a}\utpsi_{b\dot\alpha}-\unabla_{\alpha b}\utpsi_{a\dot\alpha}\,.\label{eq:phi_tpsi_tpsi_jacobi}
\end{equation}
Using \eqref{eq:bf_constraint} and  \eqref{eq:phi_tpsi_tpsi_jacobi}, we then have
\begin{equation}
    \unabla^\alpha_{\dot\alpha}\psi^a_\alpha=-\frac{2}{3}[\utpsi_{\dot\alpha b},\uphi^{ab}]-\frac{1}{3!}\epsilon^{abcd}\unabla^\alpha_b\unabla_{\alpha c}\utpsi_{\dot\alpha d}\,.
\end{equation}
Using \eqref{eq:ff_constraint}, the last term can be written as
\begin{equation}
    -\frac{1}{3!}\epsilon^{abcd}\unabla^\alpha_b\unabla_{\alpha c}\utpsi_{\dot\alpha d}=-\frac{1}{3}[\uphi^{ab},\utpsi_{\dot\alpha b}]\,,
\end{equation}
so that we reproduce \eqref{eq:super_psi_eom}
\begin{equation}
    \unabla_{\dot\alpha}^\alpha\upsi_\alpha^a=-\frac{1}{3}[\utpsi_{\dot\alpha b},\phi^{ab}]\,.
\end{equation}

In the same way, we can use \eqref{eq:ff_constraint} to obtain for the fermionic derivative acting of $\upsi^a_\alpha$
\begin{equation}
    \unabla_{a\alpha}\upsi^b_\beta=\frac{1}{2}\varepsilon_{\alpha\beta}[\uphi_{ac},\uphi^{bc}]+\frac{1}{4}\delta^b_a\uB_{\alpha\beta}\,.\label{eq:fermionic_derivative_psi}
\end{equation}
From \eqref{eq:bf_constraint}, \eqref{eq:phi_tpsi_tpsi_jacobi}, and \eqref{eq:fermionic_derivative_psi} one can straightforwardly show that
\begin{equation}
    \unabla^\beta_{\dot\alpha}\uB_{\alpha\beta}=-2\{\utpsi_{a\dot\alpha},\upsi^a_\alpha\}+\frac{1}{3}[\uphi_{ab},\unabla_{\alpha\dot\alpha}\uphi^{ab}]\,,
\end{equation}
thus reproducing \eqref{eq:super_B_eom}. In the following, we'll also need the first and second fermionic derivatives of $\uB_{\alpha\beta}$. The first derivative can be obtained via \eqref{eq:ff_constraint} and reads
\begin{equation}
    \unabla^\beta_a\uB_{\alpha\beta}=-6[\uphi_{ab},\upsi^b_\alpha]\,,\label{eq:fermionic_derivative_B}
\end{equation}
so that acting with a further derivative and using \eqref{eq:fermionic_derivative_psi} we obtain
\begin{equation}
    \unabla^\alpha_{[a}\unabla^\beta_{b]}\uB_{\alpha\beta}=-6\epsilon_{abcd}\{\upsi^c_\alpha,\upsi^{d\alpha}\}-6[\uphi_{c[a},[\uphi^{cd},\uphi_{b]d}]]\,.\label{eq:double_fermionic_derivative_B}
\end{equation}

We can finally derive the equations of motion for the positive-helicity spinors and the scalars. Starting with the spinors, the Jacobi identity for $\underline\nabla_{\alpha a}$, $\underline\nabla_{\beta\dot\beta}$ and $\underline\nabla_{\gamma\dot\gamma}$ can be written as
\begin{equation}
        2\unabla_a^{\beta}\uF_{\beta\alpha}=3\unabla_\alpha^{\dot\alpha}\utpsi_{a\dot\alpha}\,,\label{eq:F_tpsi_jacobi}\\
\end{equation}
so that \eqref{eq:F_B_lagrange_multiplier} and \eqref{eq:fermionic_derivative_B} directly give \eqref{eq:super_tpsi_eom}
\begin{equation}
    \unabla_\alpha^{\dot\alpha}\utpsi_{a\dot\alpha}=-4\lambda[\uphi_{ab},\upsi^b_\alpha]\,.
\end{equation}
Similarly, acting with $\unabla^{\alpha\dot\alpha}$ on \eqref{eq:phi_tpsi_tpsi_jacobi} and using \eqref{eq:bf_constraint} yield
\begin{equation}
    \usquare\phi_{ab}=2\{\utpsi_{\dot\alpha[a},\utpsi^{\dot\alpha}_{b]}\}-\frac{2}{3}\unabla^\alpha_{[a}\unabla^\beta_{b]}\uF_{\alpha\beta}\,.\label{eq:super_phi_eom_partial}
\end{equation}
so that using \eqref{eq:double_fermionic_derivative_B} finally gives the last missing equation of motion, namely \eqref{eq:super_phi_eom}
\begin{equation}
    \usquare\uphi_{ab}=2\{\utpsi_{\dot\alpha[a},\utpsi^{\dot\alpha}_{b]}\}+4\lambda\epsilon_{abcd}\{\upsi^c_\alpha,\upsi^{d\alpha}\}+4\lambda[\uphi_{c[a},[\uphi^{cd},\uphi_{b]d}]]\,.
\end{equation}
